Vector Bosons and Jets in Proton Collisions

Events with vector bosons produced in association with jets have been extensively studied at hadron colliders and provide high-accuracy tests of the Standard Model. A good understanding of these processes is of paramount importance for precision Higgs physics, as well as for searches for new physics. In particular, associated production of $\gamma$, $W$ or $Z$ bosons with light-flavor and heavy-flavor jets is a powerful tool for testing perturbative QCD calculations, Monte Carlo event generators, and can also constrain the parametrizations used to describe the parton content of the proton. Furthermore, events with a $W$ or $Z$ boson produced with two well-separated jets can be used to distinguish between electroweak and strong production mechanisms, and to set limits on contributions of physics beyond the Standard Model. This review summarises the historical theoretical developments and the state-of-the-art in the modeling of vector-boson-plus-jet physics, while focusing on experimental results by LHC collaborations in Run-1 and Run-2, and including comparisons with recent measurements at the Tevatron.

==> extra_figures.tex <==
\section{Extra Figures}

Add here any extra figure we may want to consider.

%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\centering
\includegraphics[width=0.40\textwidth]{figures/VLF_exp/VLF_WZ/CMS_Zjets_8TeV_doublediff-SMP-14-013_Figure_039.pdf}
\includegraphics[width=0.40\textwidth]{figures/VLF_exp/VLF_WZ/CMS_Zjets_8TeV_doublediff-SMP-14-013_Figure_041.pdf}
%\includegraphics[width=0.40\textwidth]{figures/VLF_exp/VLF_WZ/CMS_Zjets_8TeV_doublediff-SMP-14-013_Figure_043.pdf}
\caption{\label{fig:CMS_WZjet_8TeV_ptN_appendix} CMS $Z$-jets at 8 TeV double differential. To show agreement data and HO QCD calculations at (N)NLO.~\cite{Khachatryan:2016crw}. 
}
\end{figure}
